Dual Mesh Convolutional Networks for Human Shape Correspondence

Convolutional networks have been extremely successful for regular data structures such as 2D images and 3D voxel grids. The transposition to meshes is, however, not straight-forward due to their irregular structure. We explore how the dual, face-based representation of triangular meshes can be leveraged as a data structure for graph convolutional networks. In the dual mesh, each node (face) has a fixed number of neighbors, which makes the networks less susceptible to overfitting on the mesh topology, and also al-lows the use of input features that are naturally defined over faces, such as surface normals and face areas. We evaluate the dual approach on the shape correspondence task on theFaust human shape dataset and variants of it with differ-ent mesh topologies. Our experiments show that results of graph convolutional networks improve when defined over the dual rather than primal mesh. Moreover, our models that explicitly leverage the neighborhood regularity of dual meshes allow improving results further while being more robust to changes in the mesh topology.

==> old_experiments.tex <==
\iffalse

\subsection{Shape Classification}

The task of shape classification consist in assigning a single class label to the entire shape, indicating what type of object it represents.

\mypar{Dataset and evaluation metrics}
We use the SHREC'11 \cite{lian2011shape} dataset which consists of 600 3D shapes divided into 30 different categories with 20 shapes each. 
We use the experimental setup from \cite{ezuz2017gwcnn, hanocka19tog} and split the data to create two sets: Shrec16 (16 train/4 test) and Shrec10 (10 train/10 test). 
We train models over the original meshes, as well as the lower-resolution meshes from \cite{hanocka19tog}.
Unless specified otherwise, we report the mean  classification accuracy across  3 randomly generated splits.

\mypar{Network architectures}
We use the following architecture given a mesh with $N_f$ faces, $N_i$ input features and $N_t$ target classes:
Input($N_f$, $N_i$) - DualConv($N_f$, 32) - DualConv($N_f$, 64) - DualConv($N_f$, 128) - Dual($N_f$, 256) - GlobalAvgPool - Linear(256, 100) - Linear(100, $N_t$) - Output($N_t$)


\mypar{Experimental results}
In Table \ref{tab:shrec_classification_resolution}, we compare the accuracy using our method on a particular split of the original meshes and the reduced (lower resolution) meshes from \cite{hanocka19tog}. We observe that the results are significantly better on the reduced meshes. We use these reduced meshes for the rest of our experiments.

In Table \ref{tab:shrec_classification_inputs}, we report results obtained using DualConvMax with different combinations of input features. We observe that the combination of inputs which include rotation/translation invariant features such as Face/Dihedral/Area/DistCM perform much better.

In Table \ref{tab:shrec_classification_sota}, we mention the state-of-the-art reported in \cite{hanocka19tog}.

\begin{table}[]
    \centering
    % \resizebox{\columnwidth}{!}{
    \begin{tabular}{lccc}
        \toprule
        Input & Original & Reduced \\
        \midrule
        XYZ & $69.2\%$ & $74.2\%$ \\
        Normal+Area+DistCM & $95.8\%$ & $97.5\%$ \\
        Face+Dihedral & $89.2\%$ & $99.2\%$ \\
        \bottomrule
    \end{tabular}
    % }
    \caption{SHREC'11 Classification: DualConvMax on the original and lower resolution version of the meshes. The results are reported on a particular split of Shrec16.
    }
    \label{tab:shrec_classification_resolution}
\end{table}

\begin{table}[]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lccc}
        \toprule
        Input & Shrec16 & Shrec10 \\
        \midrule
        XYZ & $66.7\%$ & $57.3\%$ \\
        Normal+Area+DistCM & $94.2\%$ & $91.3\%$ \\
        % Face+Dihedral & $96.4\%$ & $94.0\%$ \\
        Face+Dihedral+Area+DistCM & $97.3\%$ & $\textbf{94.4\%}$ \\
        XYZ+DistCM+Normal+Dihedral+Area & $\textbf{98.1\%}$ & $92.9\%$ \\
        \bottomrule
    \end{tabular}}
    \caption{SHREC'11 Classification with different input features for DualConvMax. The results are averaged over 3 randomly generated splits.
    }
    \label{tab:shrec_classification_inputs}
\end{table}


\begin{table}[]
    \centering
    % \resizebox{\columnwidth}{!}{
    \begin{tabular}{lccc}
        \toprule
        Method & Shrec16 & Shrec10 \\
        \midrule
        MeshCNN \cite{hanocka19tog} & $98.6\%$ & $91.0\%$ \\
        GWCNN & $96.6\%$ & $90.3\%$ \\
        GI & $96.6\%$ & $88.6\%$ \\
        SN & $48.4\%$ & $52.7\%$ \\
        \bottomrule
    \end{tabular}
    % }
    \caption{SHREC'11 Classification: State of the Art.
    }
    \label{tab:shrec_classification_sota}
\end{table}


\subsection{Shape Segmentation}

The Human Body Segmentation \cite{maron2017convolutional} dataset contains 370 training meshes (SCAPE, FAUST, MIT and Adobe Fuse) and 18 testing meshes (SHREC). Each mesh is manually segmented into eight labels, which are provided per face. 

We normalize the data by first re-scaling all the meshes to 200cm geodesic diameter and then translating them to have zero mean. We use data augmentation by rotating the mesh along a randomly chosen axis and angle during training.

\jakob{Are the random rotations only applied at train, or also at test? What is the impact of the random rotations? Are cited results from other methods also confronted with random rotations at train and/or test? }

\nitika{Random rotations are only added during train. Most of the sota use random rotations during training, the remaining don't mention in the papers. The test set remains unchanged. Added the impact of rotations in Table \ref{tab:segmentation_rotations}}

\nitika{SOTA methods mostly use U-Net architecture for human body segmentation.}


\begin{table}[]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lcc}
        \toprule
        Method & Input & Accuracy \\
        \midrule
        Mesh CNN \cite{hanocka19tog} & Dihedral+FaceAngles+EdgeRatio & $92.3\%$  \\
        Toric Cover\cite{maron2017convolutional} & WKS, AGD, curv & $88.0\%$ \\
        PointNet++ \cite{qi17nips} & XYZ & $90.77\%$ \\
        MDGCNN \cite{poulenard2018multi} & SHOT & $89.47\%$ \\
        GCNN \cite{masci15iccvw} & SHOT & $86.4\%$ \\
        DynGraphCNN \cite{wang2019dynamic} & XYZ & $89.72\%$ \\
        SurfaceNet \cite{haim2019surface} & XYZ & $91.31\%$ \\
        ZerNet \cite{sun2018zernet} & XYZ & $88.7\%$ \\
        % \midrule
        % PointNet++ (Replicate) & XYZ & $77.8\%$ \\
        % \midrule
        % DualConvMax & XYZ & $58.6\%$ \\
        % DualConvMax & XYZ+Normal & $68.6\%$ \\
        \bottomrule
    \end{tabular}}
    \caption{Human Body Segmentation results using our model and state-of-the-art models.}
    \label{tab:my_label}
\end{table}

\begin{table}[]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lcc}
        \toprule
        Input & Normalized & Normalized+Rotations\\
        \midrule
        XYZ & $52.4\%$ & $63.8\%$ \\
        XYZ + Normal + Area & $55.3\%$ & $67.7\%$ \\
        XYZ+Normal+Area+Dihedral+DistCM & $59.1\%$ & $74.9\%$ \\
        Normal + Area + DistCM & $56.8\%$ & $62.9\%$ \\
        Dihedral + Area + DistCM & $59.9\%$ & $59.9\%$ \\
        \bottomrule
    \end{tabular}}
    \caption{Human Body Segmentation: Comparison of results using the original, normalized and data augmentation using random rotations during training.}
    \label{tab:segmentation_rotations}
\end{table}

\fi

